AgenticSTS: A Bounded-Memory Testbed for Long-Horizon LLM Agents

Memory for a long-horizon LLM agent is a contract about what each future decision is allowed to see. The simplest contract appends past observations, tool calls, and reflections to every prompt, which makes prior context easy to access but also turns it into a jumbled mixture in which the effect of any single memory component is hard to isolate. We introduce and instrument an alternative bounded contract: every decision is made from a fresh user message assembled by typed retrieval, with no raw cross-decision transcript appended. The prompt thus stays bounded across runs of any length, and any single layer can be ablated in isolation. We instantiate the contract in Slay the Spire 2, a closed-rule stochastic deck-building game whose runs require hundreds of tactical and strategic decisions. A public online benchmark of frontier LLMs on the same game reports zero wins at the lowest difficulty across five configurations, and the developer-reported human win rate at the same difficulty is 16%; the task is hard but not saturated. Within our harness, a fixed-A0 ablation shows the largest observed difference when triggered strategic skills are enabled: the no-store baseline wins 3/10 games and adding the skill layer 6/10. At this sample size the comparison is directional rather than statistically decisive (Fisher exact p\approx0.37); a cross-backbone probe and public accumulating-context baselines are reported as operational comparisons rather than controlled tests of the contract variable itself. We release a reproducible testbed: 298 completed trajectories with condition tags, frozen memory/skill snapshots, prompt records, and analysis scripts -- an agent design and a validated, reusable methodology for studying how explicit memory layers shape long-horizon LLM-agent decisions.

==> sec/11.ethics.tex <==
% ============================================
% Ethical Considerations
% ============================================
% No \section here — main.tex provides "\section*{Ethical Considerations}".

\paragraph{Subject of study.}
The agent acts only inside a single-player video game on a community
mod. No human subjects are involved, and the project collects no
personal data. We cite aggregate public community statistics and
public repository metadata, but do not redistribute user-level
community runs.

\paragraph{Game and mod licensing.}
\stspad{} is a commercial title, and the surrounding mod ecosystem
includes open-source projects such as STS2MCP, AI-Spire,
HermesBridge, and CharTyr. The artifact records community-mod
ancestry and license notes, including the CharTyr STS2 mod
\citep{chartyr-sts2-2026}, without redistributing game asset dumps.
Game names, screenshots, and textual references throughout this paper
and the released artifact are used for research documentation only;
all rights to the underlying game and its content remain with the
rights holders, and verbatim game-string tables are regenerated locally
rather than redistributed.

\paragraph{Reproducibility and data sharing.}
We release run logs, frozen $L_4{+}L_5$ artifacts, configuration
snapshots, and analysis scripts in a separate public archive with
license and provenance notes (\S\ref{sec:methodology:repro}). The
archive contains derived fields and local scripts, not a
redistributable copy of the game. It excludes scraped human dialogue,
model weights, copyrighted raw art, and game asset dumps.

\paragraph{Use of AI assistance.}
LLM systems were used for drafting and editing assistance. The
authors verified the experimental results, statistical analyses,
architecture choices, and interpretations against frozen logs and
scripts. LLM systems were not used to generate or alter raw logs or
to fabricate numerical results.

\paragraph{Risk of dual use.}
Bounded retrieval and skill write-back are general agent capabilities.
The single-player game setting has low direct harm. Deployment in
domains with real-world actions would require separate safety review,
logging, and write-gate controls.

